FanOutQA: A Multi-Hop, Multi-Document Question Answering Benchmark for Large Language Models

One type of question that is commonly found in day-to-day scenarios is ``fan-out'' questions, complex multi-hop, multi-document reasoning questions that require finding information about a large number of entities. However, there exist few resources to evaluate this type of question-answering capability among large language models. To evaluate complex reasoning in LLMs more fully, we present FanOutQA, a high-quality dataset of fan-out question-answer pairs and human-annotated decompositions with English Wikipedia as the knowledge base. We formulate three benchmark settings across our dataset and benchmark 7 LLMs, including GPT-4, LLaMA 2, Claude-2.1, and Mixtral-8x7B, finding that contemporary models still have room to improve reasoning over inter-document dependencies in a long context. We provide our dataset and open-source tools to run models to encourage evaluation at https://fanoutqa.com

==> utils.tex <==
\usepackage{xcolor}
\usepackage{xifthen}
\newcommand\todo[1]{
    \textcolor{red}{
        \ifthenelse{\isempty{#1}}
            {TODO}
            {TODO: #1}
    }
}

\newcommand{\dagsuper}[0]{\textsuperscript{\textdagger}}
\newcommand{\starsuper}[0]{\textsuperscript{*}}

\newcommand\zhu[1]{\textcolor{blue}{#1}}

